Activation-Deactivation: A General Framework for Robust Post-hoc Explainable AI

Perturbation-based explainability methods face criticism due to their reliance on out-of-distribution mutants. This raises doubts about the quality of the explanations. In this paper, we introduce a novel forward pass paradigm, Activation-Deactivation (AD), which obviates the need for perturbation of the input. AD replaces perturbation of input features with switching off parts of the model corresponding to to the intended perturbations. We implement ConvAD, an AD approximation algorithm for CNNs. ConvAD is a drop-in mechanism that can be easily added to any trained CNN and, without any additional training, generates more robust and more transferable explanations. We provide evaluation results across multiple architectures, datasets, methods and perturbation strategies, demonstrating the superior quality of ConvAD compared to the SOTA.

==> Figures/abstract_fig.tex <==
\begin{figure}
    \centering % Center the entire figure

    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/test_color_ibex_AD.png}
        \caption{AD}
        \label{fig:ad_goat}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/test_color_ibex_mask_min.png}
        \caption{Min}
        \label{fig:min_goat}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/test_color_ibex_mask.png}
        \caption{Zero}
        \label{fig:zero_goat}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/test_color_ibex_mask_avg.png}
        \caption{Avg}
        \label{fig:avg_goat}
    \end{subfigure}
    \begin{subfigure}{0.18\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/test_color_ibex_mask_max.png}
        \caption{Max}
        \label{fig:max_goat}
    \end{subfigure}
    \caption{Placeholder caption}
    \label{fig:abstract_fig}
\end{figure}

==> Figures/attribution.tex <==

\begin{tikzpicture}%[show grid = true]
    \begin{scope}[scale=0.5,xshift=-5cm]
        \matrix[matrix of nodes, nodes={minimum size=0.7cm, draw, anchor=center},
            row sep=-\pgflinewidth, column sep=-\pgflinewidth](mygrid) {%
            1 & 0 & 1 & 1 \\
            1 & 0 & 1 & 1 \\
            1 & 1 & 1 & 1 \\
            1 & 1 & 1 & 1\\
        };
        \node[draw=red,fill=red,fill opacity=0.1,rectangle,inner sep=0pt,minimum width=1.4cm,minimum height=1.4cm]
            (window) at (-1.4, 1.4) {};
    \end{scope}
 
    \begin{scope}[scale=0.5,xshift=5cm]
        \matrix[matrix of nodes, nodes={minimum size=0.7cm, draw, anchor=center},
            row sep=-\pgflinewidth, column sep=-\pgflinewidth](mygrid) {%
            0.50& 0.50 & 1.00 \\
            0.75 & 0.75 & 1.00 \\
            1.00 & 1.00 & 1.00 \\
        };
        
        \node (layer) at (0, 3) {\Large{$M'$}};
        
        \node[draw=blue,fill=blue,fill opacity=0.1,rectangle,inner sep=0pt,minimum width=0.85cm,minimum
        height=0.7cm] (dot) at (-1.70, 1.4) {};
    \end{scope}

    \draw[-Triangle,very thick, blue] (window.north) to [out=45, in=135] (dot.north);
    \node[blue] (con) at (-1,2.7) {\Large{$\Phi_i$}};

   % \draw[-Triangle,very thick,blue,bend left] (dot.west) to [out=45,in=135] (window.east) {}; %{$\mathit{pos}_{N}$};
   % \node[blue] (pos) at (0, -0.7) {\large{$\Phi_{i}$}};

\end{tikzpicture}
